Fine-grained Domain Adaptive Crowd Counting via Point-derived Segmentation

Due to domain shift, a large performance drop is usually observed when a trained crowd counting model is deployed in the wild. While existing domain-adaptive crowd counting methods achieve promising results, they typically regard each crowd image as a whole and reduce domain discrepancies in a holistic manner, thus limiting further improvement of domain adaptation performance. To this end, we propose to untangle \emph{domain-invariant} crowd and \emph{domain-specific} background from crowd images and design a fine-grained domain adaption method for crowd counting. Specifically, to disentangle crowd from background, we propose to learn crowd segmentation from point-level crowd counting annotations in a weakly-supervised manner. Based on the derived segmentation, we design a crowd-aware domain adaptation mechanism consisting of two crowd-aware adaptation modules, i.e., Crowd Region Transfer (CRT) and Crowd Density Alignment (CDA). The CRT module is designed to guide crowd features transfer across domains beyond background distractions. The CDA module dedicates to regularising target-domain crowd density generation by its own crowd density distribution. Our method outperforms previous approaches consistently in the widely-used adaptation scenarios.

==> network/sec_experiments.tex <==
\vspace{-2mm}\section{Experiments}\label{sec:application}\vspace{-2mm}
We conduct extensive experiments to evaluate our approach on several crowd benchmarks: ShanghaiTech PartA \cite{zhang2016single}, UCF-QNRF \cite{idrees2018composition}, UCF\_CC\_50 \cite{idrees2013multi}, and JHU-CROWD++ \cite{sindagi2019pushing}, \cite{sindagi2020jhu}.
We compare our approach against other weakly-supervised counting methods. Note that, compared to the existing weakly-supervised methods, our ranking-based model requires weaker supervision.
%The purpose is to verify the proposed method can achieve superior performance over other weakly-supervised counting methods, with a more-weakly learning setting, and understand the influence of settings of our method.
In this section, we first describe the implementation details and evaluation metrics. Then, we compare and evaluate our method with the peer weakly-supervised state-of-the-art methods. Last, we perform comprehensive ablation studies to delve into our model.
\vspace{-2mm}

\subsection{Implementation Details and Metrics}
\textbf{Implementation Details.} We implement our model using Pytorch \cite{paszke2019pytorch}. The network backbone used in our experiment is CSRNet \cite{li2018csrnet}. Apparently, the backbone can also be replaced by other CNN-based counting model. The proposed network is trained using Adam solver \cite{kingma2014adam} as the optimizer with a mini-batch size of 1. The learning rate is set to 5e-5. Except for the ablation study, the margin of SVM in our methods is set to 0.5. Since the datasets include some high-resolution (HR) images, we downsample them to the resolution of less than $700 \times 800$.

\textbf{Evaluation Metrics.}
There are two metrics widely used to evaluate the performance of crowd counting. Mean Absolute Error (MAE) implies count estimation accuracy, which is formally defined as,
\begin{align}
MAE = \frac{1}{\mathcal{N}} \sum_{i=1}^{\mathcal{N}}|c_i - c_i^{GT}|,
\end{align}
%$$ MAE = \frac{1}{\mathcal{N}} \sum_{i=1}^{\mathcal{N}}|c_i - c_i^{GT}|,$$
where $\mathcal{N}$ is the number of images in the testing set. $c_i$ is the predicted count for $i$-th image, while its actual count is $c_i^{GT}$.
Mean Squared Error (MSE) is the metric for variance of counting estimation to reflect the robustness of prediction, which is defined as,
\begin{align}
MSE = \sqrt{\frac{1}{\mathcal{N}} \sum_{i=1}^{\mathcal{N}}(c_i - c_i^{GT})^2}.
\end{align}
%$$ MSE = \sqrt{\frac{1}{\mathcal{N}} \sum_{i=1}^{\mathcal{N}}(c_i - c_i^{GT})^2}.$$
\textbf{\rll{Anchoring Mapping.}}
\rll{During inference, to evaluate the proposed ranking method, the scaling mapping function $S:v\rightarrow y$ from potential scores to real count numbers can be learned by linearly fitting the images in the counting anchor set, where $\{v, y\}$ is paired and known.}

\begin{table*}[t]
	\centering
	\tiny
	\tabcolsep=0.05cm
	\setlength\arrayrulewidth{1.0pt}
	\caption{Comparison of our proposed method with baselines and related methods on ShanghaiTech Part A \cite{zhang2016single} and UCF-QNRF \cite{idrees2018composition}. ``label level'' refers to the supervision level of training. \ding{52} means the model employs all the labels under the corresponding level of supervision, and \ding{70} means the model employs a few labels at this supervision level. $*$ indicates the $0.1\%$ of the parameters are tuned with location-level supervision. \rll{Note that, \textit{Ours++ (Fully)} exploits full count labels as supervision, and ranking labels can be auto-generated from count label without extra annotating effort.} The best results in weakly-supervised setting are highlighted in \rbf{red}.}
	\begin{tabular}{c||x{1.1cm}x{0.8cm}x{1.0cm}x{1.05cm}|x{0.75cm}x{0.7cm}|x{0.75cm}x{0.7cm}}
		\toprule
		&\multicolumn{4}{c|}{\textbf{Label level}} & \multicolumn{2}{c|}{\textbf{ST PartA}\cite{zhang2016single}} & \multicolumn{2}{c}{\textbf{UCF-QNRF}\cite{idrees2018composition}} \\
		\midrule
		\textbf{Method} & \textbf{Location} & \textbf{Count} & \textbf{Ranking} & \textbf{No label}& \textbf{MAE$\downarrow$} & \textbf{MSE$\downarrow$} & \textbf{MAE$\downarrow$} &\textbf{MSE$\downarrow$} \\
		\midrule
		MCNN \cite{zhang2016single} (2016) & \ding{52} &  &  &  & 110.2 & 173.2 & 277.0 & 426.0 \\
		Switching-CNN \cite{sam2017switching} (2017) & \ding{52} &  &  &  & 90.4 & 135.0 & 228.0 & 445.0\\
		CSRNet \cite{li2018csrnet} (2018) & \ding{52} &  &  &  & 68.2 & 115.0 & 119.2 & 211.4 \\
		CAN \cite{liu2019context} (2019) & \ding{52} &  &  &  & 62.3 & 100.0 & 107.0 & 183.0 \\
		ADSCNet \cite{bai2020adaptive} (2020) & \ding{52} &  &  &  & {55.4} & {97.7} & {71.3} & {132.5} \\
		\midrule
		GWTA-CCNN \cite{sam2019almost} (2019) & $*$ &  &  & \ding{52} & 154.7 & 229.4 & - & -\\
		CSS-CCNN \cite{sam2020completely} (2020) &  &  &  & \ding{52} & 207.3 & 310.1 & 442.4 & 721.6 \\
		IRAST (Label only) \cite{liu2020semi} (2020) & \ding{70} &  &  &  & 98.3 & 159.2 & 147.7 & 253.1  \\
		IRAST \cite{liu2020semi} (2020) & \ding{70} &  &  & \ding{52} & 86.9 & 148.9 & 135.6 & 233.4 \\
		CCLS \cite{yang2020weakly} (2020) &  & \ding{52} &  &  & 104.6 & 145.2 & - & - \\
		\midrule
		CSRNet(Count label only) &  & \ding{52} &  &  & 85.6 & 128.1 & 149.0 & 245.3 \\
		CSRNet(Count label only)+L2R \cite{liu2018leveraging} &  & \ding{52} &  &  & 84.91 & 125.2 & 144.6 & 238.2 \\
		Ours &  &  & \ding{52} &  & 93.4 & 142.5 & 165.3 & 277.7  \\
		Ours++ &  & \ding{70} & \ding{52} &  & 91.6 & 138.5 & 158.7 & 266.7  \\
		Ours++ (Fully) &  & \ding{52} & \ding{52} &  & \rbf{76.9} & \rbf{113.1} & \rbf{133.0} & \rbf{218.8} \\
		\bottomrule
	\end{tabular}
	\label{table:1}\vspace{-5mm}
\end{table*}


\subsection{Comparison with State-of-the-arts}
Compared with previous weakly-supervised counting methods, our supervision scheme is unique, which requires less supervision information. Here, we mainly compare the proposed methods with other approaches with diverse supervised settings. Our comparison evaluation is conducted on ShanghaiTech PartA \cite{zhang2016single} and UCF-QNRF \cite{idrees2018composition} datasets.
\vspace{-1mm}

\textbf{ShanghaiTech Part A Dataset.}
ShanghaiTech Part A dataset \cite{zhang2016single} is a large-scale crowd counting dataset, which is composed of 482 images with 244,167 annotated persons. The training set includes 300 images with 162,707 annotated persons, and the remaining 182 images are for testing. The images are captured from the Internet and the number of the humans ranges from 33 to 3139 per image. Following the assumption of glance annotation, the available training ranking pairs are 24,386. Due to our transitive automatic labeling, the times of manually annotating ranking pairs is reduced to 16,194. And we randomly pick up 50 images to set up the counting anchor set, which varies from different crowd density levels in the training set. In total, the number of ranking pairs is only $1/10$ of location-based labels. Adding the labeling efforts of counting anchor set, the total labeling amount is around 1/4 of the original labels on ShanghaiTech Part A dataset.
\vspace{-1mm}

\textbf{UCF-QNRF Dataset.}
The UCF-QNRF dataset \cite{idrees2018composition} contains 1,535 images with counts varying from 49 to 12865 including 1,251,642 annotated heads, thus the average count is around 815 per image. The training set includes 1,201 images, and 334 images are for testing. We also randomly pick up 70 images from different range of density as the counting anchor set. Owing to the huge data size, the number of available ranking pairs is exploded, thus it is intractable to annotate all pairs in the real world. To handle the problem, the hyper-parameter $\mathcal{N}_{sim}$ is provided to simulate the number of annotated ranking pairs when training for ranking. Here we set $\mathcal{N}_{sim} = 48,000$, which means the given set $P$ with size 48,000 is fixed before training and these pairs are available training samples.
\vspace{-1mm}

\textbf{Categories of Crowd Counting Methods.}
Generally, the supervision of the evaluation methods can be roughly categorized from laborious to effortless as four levels, location level, count level, ranking level and no label:
\begin{itemize}
	\item \textit{Location level} supervision relies on location-based density maps as the optimizing objective. For a dense-scene crowd image, it requires a lot of effort to complete the annotation of hundreds of locations.
	\item \textit{Count level} supervision is based on crowd count numbers without the location supervision. There is no many labels but one-by-one manual counting is required.
	\item \textit{Ranking level} supervision is a subjective ranking label for pair-wise images and the label can be conducted only at a glance.
	\item \textit{No label} supervision is not to use any annotated label, only use raw crowd images for input.
\end{itemize}

\textbf{Experimental Results.} In experiments, we apply several variants of our proposed method for comparison. Particularly, the model trained only with ranking labels is denoted as \textit{Ours}, whereas \textit{Ours++} refers to the model that is trained with the ranking and cost-free regression labels from the counting anchor set. Besides, \textit{Ours++ (Fully)} attaches all training images with count label for regression along with ranking label for ranking.

The quantitative comparison with the state-of-the-art methods on these two datasets is presented in Table~\ref{table:1}. The fully-supervised location-level methods are listed in the first part of table, and the weakly-/semi-/un-supervised methods for comparision are listed in the second part. The performance of the proposed method and compared baselines are at the bottom. \textit{CSRNet (Count label only)} represents the regression-based baseline supervised only by count labels. \textit{CSRNet (Count label only) + L2R \cite{liu2018leveraging}} is to add "cropping rank" supervision for the above label-only model. Note that these comparative weakly-supervised methods, \eg, IRAST \cite{liu2020semi}, CCLS \cite{yang2020weakly}, and our proposed method are also based on the same feature extractor, CSRNet \cite{li2018csrnet}, for the fair comparison. As observed, the proposed method outperforms the other competing methods with similar supervision level on the benchmarks.


\begin{figure}[t]
	\centering
	\setlength{\tabcolsep}{1pt}
	\begin{tabular}{>{\centering\arraybackslash\hspace{0pt}}p{.040\linewidth}
			>{\centering\arraybackslash\hspace{0pt}}p{.265\linewidth}
			>{\centering\arraybackslash\hspace{0pt}}p{.265\linewidth}
			>{\centering\arraybackslash\hspace{0pt}}p{.265\linewidth}}
		
		
		\rotatebox{90}{\small{\centering{ST PartA}}}&
		\includegraphics[width=\linewidth]{./figs/3_visualize/ST_partA_test_IMG24_553_.jpg}&
		\includegraphics[width=\linewidth]{./figs/3_visualize/ST_partA_test_IMG24_553_645_.png}&
		\includegraphics[width=\linewidth]{./figs/3_visualize/ST_partA_test_IMG24_553_609_.png}\\
		
		\rotatebox{90}{\small{\centering{UCF-QNRF}}}&
		\includegraphics[width=\linewidth]{./figs/3_visualize/UCF-QNRF_train_IMG894_3105_.jpg}&
		\includegraphics[width=\linewidth]{./figs/3_visualize/UCF-QNRF_train_IMG894_3105_3620_.png}&
		\includegraphics[width=\linewidth]{./figs/3_visualize/UCF-QNRF_train_IMG894_3105_3504_.png}\\
		&Input & Ours & Ours++ (Fully)
	\end{tabular}
	\vspace{-3mm}\caption{Qualitative visualization of predicted density maps on two examples from ShanghaiTech PartA and UCF-QNRF by our methods. It is shown that ranking-based methods are quite good at distinguishing the crowd regions.}\vspace{-4mm}
	\label{fig:visualize}
\end{figure}


As shown in Table~\ref{table:1}, it is clear that our method outperforms the weakly-supervised regression method, CCLS \cite{yang2020weakly}, the state-of-the-art method with the same supervision level and our annotating workload is less for \textit{Ours, Ours++}. \textit{Ours++ (Fully)} achieves much less counting error than the label-only baseline due to the ranking pair supervision, and also achieves less error than the L2R supervised count label regression model. Thus, it demonstrates that ranking labels are of great use for regression at the count level supervision. Moreover, the performance of \textit{Ours++ (Fully)} is the best in weakly-supervised setting on MAE and MSE, and even close to location level baseline, CSRNet \cite{li2018csrnet}.
We visualize the density maps delivered from the last layer from network as illustrated in Fig~\ref{fig:visualize}. Although there is no location points as supervisory signals, the estimation of our approach are close to the ground truth density maps, which shows the capability of our model to identify individuals in crowds.

\vspace{-2mm}\subsection{Ablation Study}\vspace{-1mm}
%To understand the influence of various factors in our method, we conduct a series of ablation studies.
%We perform ablation studies on the hyper-parameters of our model.

\textbf{Impact of the margin on SVM.} We set hyper-parameter margin $\mathcal{M}$ to 0.5 in the previous experiments. To investigate the impact of margin, we conduct experiments on ShanghaiTech part A datasets. As shown in Table~\ref{table:2} (left), the results demonstrate setting different margin of SVM does not affect the counting performance significantly. The crowd counting performance are similar to our current results when margin is set properly, which means the proposed method is robust.

\textbf{The size of the counting anchor set.} So far, we conduct our experiment with the size of the counting anchor set $50$ (\textit{Ours++} and $300$ for \textit{Ours++(Fully)}, which is the full of ShanghaiTech Part A training set. It is unclear the performance gain is affected with varying its size during training phase. To investigate this, we conduct an experiment that applies different sizes on ShanghaiTech Part A. The results are shown in Table~\ref{table:2} (middle), we can observe an improved performance by expanding the set. It implies that the counting method based on regression labels can be incorporated into our setting and effectively boost crowd counting.

\textbf{Beyond the ``More than Twice'' Assumption.} We make a reasonable assumption that the number of people in the two images can be distinguished easily with more than twice the difference in crowd sizes between them. To explore more about the assumption, we incrementally adjusting more critical times representing for difference in numbers between a pair of images by ${1N, 1.5N, 2N, 3N}$, where $2N$ represents the setting on the above assumptions in our experiments. The results are shown in Table~\ref{table:2} (right). The results indicate that the ability of annotators to recognize and compare crowd numbers at a glance can affect the performance of the proposed method with a subjective aspect.
\begin{table}[t]
	\centering
	\scriptsize
	\tabcolsep=0.10cm
	\setlength\arrayrulewidth{1.0pt}
	\caption{Impacts of the margin $\mathcal{M}$ (left), the size of counting anchor set (middle), and the crowd number difference between a ranking image pair (right). The best results are highlighted in bold.}
	\label{table:2}
	\begin{tabular}{ccc|ccc|ccc}
		\toprule
		$\mathcal{M}$& MAE & MSE & \textbf{Set size}& MAE & MSE & \textbf{Times} & MAE & MSE\\
		\midrule
		$0$ & 94.24 & 137.24 & $|B|=10$ & 115.17 & 163.75 & $1N$ & \textbf{81.25} & \textbf{126.5}\\
		$0.1$ & 95.36 & 140.95 & $|B|=30$ & 99.18 & 137.90 & $1.5N$ & 87.27 & 134.01\\
		$0.5$ & \textbf{91.66} & 138.46 & $|B|=50$ & 91.66 & 138.46 & $2N$ & 91.66 & 138.46 \\
		$1.0$ & 91.95 & \textbf{133.45} & $|B|=80$ & 87.70 & 129.04 & $3N$ & 104.06 & 144.21 \\
		$3.0$ & 95.25 & 141.27 & $|B|=150$ & \textbf{81.09} & \textbf{120.67} & & &\\
		\bottomrule
	\end{tabular}\vspace{-2mm}
\end{table}

\subsection{Challenging Experiments}\vspace{-1mm}
%In the real-world counting works, distinct from benchmark evaluation,
\textbf{Ranking Labels in Real-world Counting.} Unlike the crowd data in benchmarks,
the real-world crowd data is often a large quantity of unlabeled crowd images, so it is infeasible to annotate all of extracted pairs.
Especially in the mid-to-late stage of training, much abundant pairs with large numerical difference almost have no effect on loss, and just consume computing power in vain. Therefore, sparse labeling is preferable for massive, wild and unlabeled crowd data.
Denote the number of labels associated with crowd image $x_i$ as $\zeta(x_i)$, and the average number of $\zeta(x_i)$ in dataset $D$ as $\zeta(D)$. (Note that only the labeled image will be included, thus $\zeta(\cdot) \geq 1$.) In short, with sufficient training samples, $\zeta(D)$ is closer to $1$, which means the labels per image are sparse. Furthermore, online labeling strategy can work well with sparse labeling. Before the start of training, the ranking pairs are labeled under the setting, $\zeta(D) = 1$. After training for some time, $\zeta(D)$ can become larger.

Practically, to verify the proposed ranking label in real scenes, we simulate the real annotation on a fixed number of real world images. They are from JHU-CROWD++ \cite{sindagi2019pushing}, which contains 1.51 million annotated heads spanning 4,372 images, and is a challenging dataset with various scenarios.
For the sparse labeling experiment, we randomly select 2,000 images forming 1,000 ranking pairs, and the sparse labeling strategy greatly reduces the number of labels per image $\zeta(D)$, from hundreds to one. In the other two experiments, we added annotated ranking pairs besides these 2,000 images with 5,000 pairs, and 25,000 pairs to verify the impact of label intensity.

The model is trained combining ranking with free regression labels ({Ours++}) from counting anchor set which size is 50. The training is on the selected images from JHU-CROWD++, and the evaluation is on the widely-used ShanghaiTech Part A dataset. As illustrated in Table~\ref{table:4}, compared with baseline of regression on the anchor set, the model with 1,000 comparision labels achieve a satisfactory performance with a few extra annotations. Adding more ranking labels leads to a slight improvement but brings heavy annotation load.

\begin{table}[t]
	\centering
	\scriptsize
	\tabcolsep=0.10cm
	\setlength\arrayrulewidth{1.0pt}
	\caption{The effect of ranking label in the simulated real-world counting.}
	\label{table:4}
	\begin{tabular}{c||cc}
		\toprule
		\textbf{Setting} & \textbf{MAE} & \textbf{MSE} \\
		\midrule
		Baseline & 130.5 & 201.4 \\
		Ours++ (1,000 pairs) & 114.9 & 177.9 \\
		Ours++ (5,000 pairs) & 108.2 & 153.5 \\
		Ours++ (25,000 pairs) & 106.4 & 148.2 \\
		\bottomrule
	\end{tabular}\vspace{-4mm}
\end{table}

\textbf{{Cross Datasets.}}
We conduct experiments to demonstrate the generalizability of our method across different data domains. The model is trained on one dataset of a source domain and evaluated on another dataset as a target domain. The results are demonstrated in Table~\ref{table:3}. We can observe that the proposed method generalizes well to the unseen evaluation datasets. Specially, the proposed method can be comparable or even slightly better than the location-level supervised methods.
%, though the evaluation performance on self dataset is inferior to partial methods, \eg, SPN \cite{xu2019learn}. This confirms the generalization of the proposed strategy.
\begin{table}[t]
	\centering
	\scriptsize
	\tabcolsep=0.10cm
	\setlength\arrayrulewidth{1.0pt}
	\caption{Cross dataset experiments on the ShanghaiTech Part A, UCF-QNRF and UCF\_CC\_50 datasets for demonstrating the generalization of different methods.}
	\label{table:3}
	\begin{tabular}{c||cc|cc|cc}
		\toprule
		& \multicolumn{2}{c|}{\tiny{\textbf{ST PartA $\rightarrow$ UCF-QNRF}}} & \multicolumn{2}{c|}{\tiny{\textbf{UCF-QNRF $\rightarrow$ ST PartA}}} & \multicolumn{2}{c}{\tiny{\textbf{ST PartA $\rightarrow$ UCF\_CC\_50}}} \\
		\midrule
		\textbf{Method} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} & \textbf{MAE} & \textbf{MSE} \\
		\midrule
		MCNN \cite{zhang2016single} & - & - & - & - & 397.7 & 624.1  \\
		L2R \cite{liu2018leveraging} & - & - & - & - & 337.6 & 434.3  \\
		SPN \cite{xu2019learn} & 236.3 & 428.4 & 87.9 & 126.3 & 368.3 & 588.4  \\
		Ours++ & 246.1 & 485.4 & 99.2 & 141.1 & 372.6 & 593.5 \\
		Ours++(Fully) & 204.8 & 412.2 & 88.7 & 127.8 & 324.1 & 435.7 \\
		\bottomrule
	\end{tabular}\vspace{-2mm}
\end{table}

\begin{figure}[t]
	\centering
	\setlength{\tabcolsep}{1pt}
	\begin{tabular}{>{\centering\arraybackslash\hspace{0pt}}p{.410\linewidth}
			>{\centering\arraybackslash\hspace{0pt}}p{.386\linewidth}}
		\includegraphics[width=\linewidth]{./figs/4_fitting_1.png} &
		\includegraphics[width=\linewidth]{./figs/4_fitting_2.png}
	\end{tabular}\vspace{-3mm}
	\caption{Accuracy (\%) of each crowd number range in the proposed models and baseline.}
	\label{fig:fitting}\vspace{-5mm}
\end{figure}

\textbf{{Varied Degrees of Congestion.}}
We further evaluate the proposed methods for different degrees of crowd congestion. We observe that the comparisons of the proposed method \textit{Ours++ (Fully)} with \rll{the baseline trained on regression labels only.} It turns out that, with more people (e.g., crowd number \textgreater 1,000), \textit{Ours++} and \textit{Ours++ (Fully)} can achieve better performance. Thus, our model can well be adapted in dense scenes.
We achieve similar results on UCF-QNRF dataset as well. The proposed method \textit{Ours++ (Fully)} outperforms the baseline especially in dense scenes, as shown in Fig~\ref{fig:fitting}.
\vspace{-1mm}


